Unpacking Security Scanners for GitHub Actions Workflows

GitHub Actions is a widely used platform to automate the build and deployment of software projects through configurable workflows. As the platform's popularity grows, it also becomes a target of choice for software supply chain attacks. These attacks exploit excessive permissions, ambiguous versions or the absence of artifact integrity checks to compromise the workflows. In response to these attacks, several security scanners have emerged to help developers harden their workflows. In this paper, we perform the first systematic comparison of 9 GitHub Actions Workflows security scanners. We compare them regarding scope (which security weaknesses they target), detection capabilities (how many weaknesses they detect), accuracy (how well their findings match manually confirmed weaknesses), and performance (how long they take to scan a workflow). In order to compare the scanners on a common ground, we first establish a classification of 10 common security weaknesses that can be found in GitHub Actions Workflows. Then, we run the scanners against a curated set of 2,722 workflows. Our study reveals that static scanners for GitHub Actions Workflows are very diverse, with both general purpose and focused scanners. More importantly, we provide evidence that these scanners implement fundamentally different analysis strategies, leading to major gaps regarding the nature and the number of reported security weaknesses. Based on this empirical evidence we make actionable recommendations for developers to harden their GitHub Actions Workflows.

==> Unpacking_Security_Scanners/old.tex <==
% old RQ2 poutine zizmor >>

\poutine and \zizmor mostly target the same common weaknesses. Yet, the two scanners implement significantly different strategies to detect the weaknesses, which explains many of their differences. For Artifact Integrity Weaknesses (AIW) come from the scanners focusing on the integrity of different workflow assets: \poutine flags checked-out content that may later be executed, including local actions; \zizmor looks for risks around uploaded artifacts, credential persistence, and cache reuse, sometimes including low-confidence detections where no concrete artifact or cache risk materializes. 
For Control Flow Weakness CFW, \poutine reports 6 weaknesses (among \actionlint’s detections) because it has a single rule that detects conditions which are always true. 
For Excessive Permission Weaknesses (EPW), \poutine checks permissions only in specific, high‑risk situations, such as workflows triggered by events that can receive external inputs, \zizmor applies broader rules by also checking job‑level settings and reporting any potentially unnecessary or overly broad permissions.
For GitHub Runner Compatibility Weaknesses (GRCW), \zizmor does not report any detections on our dataset. While some of its documented audits are only partially related to this category, they do not capture the compatibility issues present in our workflows.
\poutine reports also Injection Weaknesses (IW), with 107 weaknesses in 61 workflows, as it also looks for scripts that are run without proper checks and unsafe debug settings. \zizmor adopts a broader injection model, and flags any \verb|${{...}}| expansion in execution contexts and treats writes to \texttt{GITHUB\_ENV}/\texttt{GITHUB\_PATH} as sinks. This typically yields more IW detections for \zizmor at the cost of more low-risk flags.
\poutine is the only scanner that identifies Known Vulnerable Component Weaknesses (KVCW), by recognizing references to known vulnerable actions or versions, \zizmor does not detect any of these weaknesses despite their documentation mentioning these weaknesses. This demonstrates how some security weaknesses can go entirely unnoticed depending on which scanner is used and emphasizes the importance of complementary scanner coverage. 
\zizmor reports a small number of HGW findings as well, but these are limited to a narrow set of best-practice recommendations rather than broad hardening coverage.
When it comes to Privileged Trigger Weakness (PTW), \poutine primarily reports PTW when it can match a concrete unsafe combination, such as a privileged or externally influenced trigger paired with risky follow-up behavior, and it may also flag cases where such triggers run in a high-trust execution environment. In contrast, \zizmor detects the presence of privileged triggers but does not analyze follow-up behavior that processes external inputs, and it typically requires explicit indicators of a high-trust environment, which can lead to missed reports when the workflow uses only custom runner labels.
The detection of Secrets Exposure Weaknesses (SEW) is concentrated in \zizmor, which reports 89 detections across 48 workflows, while \poutine report 0.  \poutine flags jobs that might implicitly expose all configured secrets or run in privileged environments where secrets could leak, but does not detect any SEW instances in this dataset. \zizmor goes beyond hardcoded values and also flags risky secret handling practices, such as passing all secrets to reusable workflows or writing secrets into environment files.
Finally, for Unpinned Dependency Weaknesses (UDW), \zizmor reports significantly fewer weaknesses (2003) than the other scanners as it excludes official GitHub-maintained actions (e.g., \texttt{actions/checkout}) from its pinning rules, focusing instead on third-party actions and container images. 
\poutine detects 0 findings as it searches for a very specific case of UDW: a reused action that is not pinned, and this reused action itself reuses an action that is not pinned; i.e., \poutine targets composite actions that transitively use mutable tags.


\actionlint is general-purpose workflow security scanner, but its key feature stands in a thorough validation of mainly stands out on workflow validation and control-flow reasoning. When considering the Control Flow Weakness (CFW), \actionlint reports more findings with 79 weaknesses in 45 workflows because it applies several rules to validate conditions, including checks for always-true expressions, type mismatches, and invalid syntax in control statements. 
All GitHub Runner Compatibility Weaknesses (GRCW) are also reported by \actionlint, the only scanner that explicitly validates the workflow syntax and structure. 
For Excessive Permission Weaknesses (EPW), \actionlint reports a small number of EPWs, focusing on workflows that explicitly request elevated top-level scopes such as \texttt{contents: write} and \texttt{pull-requests: write}. 
For the Injection Weakness (IW), \actionlint only looks for unsafe shell commands and old workflow commands, e.g. \texttt{::set-output}, and reports 31 weaknesses. For Secrets Exposure Weaknesses (SEW), \actionlint reports 0 findings, as it only detects simple hardcoded credential patterns, which are not present in the analyzed workflows.



\scorecard stands out for broad hardening and dependency hygiene checks. 
For EPW, \scorecard takes a broader view, analyzing each workflow for explicit least-privilege token hardening, which results in more findings, including workflows that omit a top-level \texttt{permissions:} declaration even when their observed job-level permissions are read-only.
\scorecard also detects a large number of Hardening Gap Weaknesses (HGW) in our benchmarkthrough workflow-level security hygiene checks, consistently flagging the absence of a SAST tool, with one detection per affected workflow. It detects HGWs in almost all workflows in our dataset (2638 of \nbworkflows).
For IW, \scorecard reports 5 weaknesses, flagging conditional script execution based on untrusted input from commit messages, a pattern that is also detected by other scanners in our dataset.
For PTW, \scorecard takes a more pattern-driven view and flags PTW when privileged triggers are used in ways that clearly enable untrusted code execution, most notably \texttt{pull\_request\_target} combined with a checkout of the incoming pull request’s code. 
Finally, \scorecard reports the highest number of UDW findings because it checks pinning beyond reused actions, including tooling dependencies such as package installers (11347).

% old RQ2 poutine zizmor <<


%taken out of fig 1
      - name: Setup Node.js 18.x
        uses: actions/setup-node@v3
        with:
          node-version: 18.x
      - name: Install in packages/excalidraw
        run: yarn
        working-directory: packages/excalidraw
        env:
          CI: true


% long version of poutine and zizmor in RQ1
\poutine and \zizmor are the most versatile scanners, with the broadest issue detection coverage. \zizmor searches for all 10 issues with 23 rules. For instance its \texttt{excessive-permissions} rule performs the Excessive Permission Issue (EPI) detection. 
This rule identifies every location in a workflow that grants overly broad repository or workflow privileges. 
It also supports Secrets Exposure Issue (SEI) with \texttt{hardcoded-container-credentials} for secrets embedded directly in container definitions, \texttt{secrets-inherit} for when secrets are implicitly passed to reusable workflows or actions, and \texttt{unredacted-secrets} for secrets that may be output without masking. These rules locate unintentional exposures of inherited secrets to untrusted contexts. Other rules for Injection Issue (II) with \texttt{github-env}, \texttt{insecure-commands}, and \texttt{template-injection} rules, which detect unsafe uses of environment variable writes, insecure shell commands, and untrusted template inputs that could allow command or workflow injection.
\poutine, covers seven issues with 13 rules and focuses specifically on third-party and supply chain risks. For example, it has a rule for Artifact Integrity Issue (AII): \texttt{untrusted\_checkout\_exec} checks for unverified or malicious repositories. 
Another rule related to Trigger Misuse Issue (TMI),  \texttt{pr\_runs\_on\_self\_hosted}, detects when pull requests are configured to run on self-hosted runners.
It implements the Known Vulnerable Component Issue (KVCI) with its \texttt{known\_vulnerability\_in\_\allowbreak build\_component} rule that flags usages of components with published CVEs. 
Unlike \zizmor, which accepts both workflow files and repositories, \poutine requires a full repository as input.  
Their configuration models also differ: zizmor.yml primarily supports the selection of specific rules or patterns, whereas .poutine.yml offers fine-grained policy controls that allow selective rule enforcement, filtering by severity or vulnerability IDs, and defining allowed runners. 
In short, \zizmor provides broad general-purpose security scanning, while \poutine prioritizes supply chain integrity with contextual checks, both targeting high-impact issues critical for helping developers prevent privilege escalation and supply chain compromises.

